The Brain Tumor Segmentation in Pediatrics (BraTS-PEDs) Challenge: Focus on Pediatrics (CBTN-CONNECT-DIPGR-ASNR-MICCAI BraTS-PEDs)

Pediatric tumors of the central nervous system are the most common cause of cancer-related death in children. The five-year survival rate for high-grade gliomas in children is less than 20%. Due to their rarity, the diagnosis of these entities is often delayed, their treatment is mainly based on historic treatment concepts, and clinical trials require multi-institutional collaborations. Here we present the CBTN-CONNECT-DIPGR-ASNR-MICCAI BraTS-PEDs challenge, focused on pediatric brain tumors with data acquired across multiple international consortia dedicated to pediatric neuro-oncology and clinical trials. The CBTN-CONNECT-DIPGR-ASNR-MICCAI BraTS-PEDs challenge brings together clinicians and AI/imaging scientists to lead to faster development of automated segmentation techniques that could benefit clinical trials, and ultimately the care of children with brain tumors.

==> Notes.tex <==
# Important notes/TODO for manuscript goes here 

Please make sure you add the following authors in the next revision of each challenge manuscript.
Verena Chung, Sage Bionetworks
Maria Diaz, Sage Bionetworks
Byrone Cole, Sage Bionetworks
James Eddy, Sage BIonetworks
Jake Albrecht, Sage Bionetworks

It would also be nice to have a consistent description of the Synapse platform: 

Synapse is a collaborative research platform that helps teams share, organize, and discuss their scientific research.  Synapse supports the capacity to create and manage community data challenges, using containerized models for secure evaluation of participant submitted methods.

 
